Safety-Critical Learning of Robot Control with Temporal Logic Specifications

Reinforcement learning (RL) is a promising approach. However, success is limited to real-world applications, because ensuring safe exploration and facilitating adequate exploitation is a challenge for controlling robotic systems with unknown models and measurement uncertainties. The learning problem becomes even more difficult for complex tasks over continuous state-action. In this paper, we propose a learning-based robotic control framework consisting of several aspects: (1) we leverage Linear Temporal Logic (LTL) to express complex tasks over infinite horizons that are translated to a novel automaton structure; (2) we detail an innovative reward scheme for LTL satisfaction with a probabilistic guarantee. Then, by applying a reward shaping technique, we develop a modular policy-gradient architecture exploiting the benefits of the automaton structure to decompose overall tasks and enhance the performance of learned controllers; (3) by incorporating Gaussian Processes (GPs) to estimate the uncertain dynamic systems, we synthesize a model-based safe exploration during the learning process using Exponential Control Barrier Functions (ECBFs) that generalize systems with high-order relative degrees; (4) to further improve the efficiency of exploration, we utilize the properties of LTL automata and ECBFs to propose a safe guiding process. Finally, we demonstrate the effectiveness of the framework via several robotic environments. We show an ECBF-based modular deep RL algorithm that achieves near-perfect success rates and safety guarding with high probability confidence during training.

==> automaton.tex <==
\begin{figure}[!t]\centering
	\subfloat[]{{
	    \scalebox{.7}{
	    	\begin{tikzpicture}[shorten >=1pt,node distance=2.5cm,on grid,auto] 
			\node[] (s_0)   {}; 
			\node[state, initial] (s_0) [above right=of s_0, label=above:$\textcolor{blue}{\{r_0\}}$]  {$s_0$};
			\node[state] (s_1) [above right=of s_0, label=above:$\textcolor{blue}{\{r_1\}}$]  {$s_1$};
			\node[state] (s_2) [below right=of s_0, label=below:$\textcolor{blue}{\{r_2\}}$]  {$s_2$};
			\path[->] 
			(s_0) edge [bend left=15] node {$\textcolor{red}{a_{01}}$} (s_1)
			(s_1) edge [bend left=15] node {$\textcolor{red}{a_{10}}$} (s_0)
			(s_1) edge [loop right] node {$\textcolor{red}{a_{11}}$} (s_1)
			(s_2) edge [loop right] node {$\textcolor{red}{a_{22}}$} (s_2)
			(s_0) edge [bend left=15] node {$\textcolor{red}{a_{02}}$} (s_2)
			(s_2) edge [bend left=15] node {$\textcolor{red}{a_{20}}$} (s_0);
			\end{tikzpicture}

			}

			}}
	\subfloat[]{{
		\scalebox{.7}{
			\begin{tikzpicture}[shorten >=1pt,node distance=2.5cm,on grid,auto] 
			\node[state,initial] (q_0)   {$q_0$}; 
			\node[state,accepting] (q_1) [above right=of q_0, label=above:$\textcolor{ForestGreen}{F_1}$]  {$q_1$};
			\node[state,accepting, label=below:$\textcolor{ForestGreen}{F_2}$] (q_2) [below right=of q_0]  {$q_2$};
			\path[->] 
			(q_0) edge [bend left=15] node {$r_1$} (q_1)
			(q_1) edge [bend left=15] node {$r_0$} (q_0)
			(q_0) edge [loop below] node {$r_0$} (q_0)
			(q_1) edge [loop right] node {$r_1$} (q_1)
			(q_2) edge [loop right] node {$r_2$} (q_2)
			(q_0) edge [bend left=15] node {$r_2$} (q_2)
			(q_2) edge [bend left=15] node {$r_0$} (q_0)
			(q_1) edge [bend left=15] node {$r_2$} (q_2)
			(q_2) edge node {$r_1$} (q_1);
			\end{tikzpicture}
			}
			}}
	$\qquad$
	\subfloat[]{{
		\scalebox{.6}{
			\begin{tikzpicture}[shorten >=1pt,node distance=3cm,on grid,auto] 
			\node[state,initial] (s_0)   {$(s_0,q_0)$}; 
			\node[state,accepting] (s_1) [above right=of s_0, label=above:$\textcolor{ForestGreen}{F_1}$]  {$(s_1,q_1)$};
			\node[state] (s_2) [below right=of s_0]  {$(s_0,q_0)$};
			\draw[blue, very thick] (1.2,-3) rectangle (3,-1.2);
			\path (3.65,0) node(x) {\textcolor{blue}{Cycle1}};
			\path (3.65,-2.1) node(x) {\textcolor{blue}{Cycle2}};
			\node[state,accepting] (s_3) [right=of s_1, label=above:$\textcolor{ForestGreen}{F_1}$]  {$(s_1,q_1)$};
			\node[state,accepting] (s_4) [right=of s_2, label=below:$\textcolor{ForestGreen}{F_2}$]  {$(s_2,q_2)$};
			\path[->] 
			(s_0) edge node {$\textcolor{red}{a_{01}^p}$} (s_1)
			(s_1) edge [bend right=15] node {$\textcolor{red}{a_{10}^p}$} (s_2)
			(s_2) edge [bend left=15] node {$\textcolor{red}{a_{01}^p}$} (s_3)
			(s_3) edge [bend left=15] node {$\textcolor{red}{a_{10}^p}$} (s_2)
			(s_3) edge [loop right] node {$\textcolor{red}{a_{11}^p}$} (s_3)
			(s_2) edge [bend left=15] node {$\textcolor{red}{a_{02}^p}$} (s_4)
			(s_4) edge [bend left=15] node {$\textcolor{red}{a_{20}^p}$} (s_2)
			(s_4) edge [loop right] node {$\textcolor{red}{a_{22}^p}$} (s_4)
			;
			\end{tikzpicture}
			}
		}}
		\caption{\label{fig:automaton} (a) PL-MDP model with the deterministic label function. (b) LDGBA of LTL formula
		$\varphi_{e}$. (c) The standard product MDP.}
	\end{figure}

==> automaton_example.tex <==
\begin{figure}[!t]\centering
	\subfloat[]{{
	    \scalebox{.7}{
	    	\begin{tikzpicture}[shorten >=1pt,node distance=2.5cm,on grid,auto] 
			\node[] (s_0)   {}; 
			\node[state, initial] (s_0) [above right=of s_0, label=above:$\textcolor{blue}{\{r_0\}}$]  {$s_0$};
			\node[state] (s_1) [above right=of s_0, label=above:$\textcolor{blue}{\{r_1\}}$]  {$s_1$};
			\node[state] (s_2) [below right=of s_0, label=below:$\textcolor{blue}{\{r_2\}}$]  {$s_2$};
			\path[->] 
			(s_0) edge [bend left=15] node {$\textcolor{red}{a_{01}}$} (s_1)
			(s_1) edge [bend left=15] node {$\textcolor{red}{a_{10}}$} (s_0)
			(s_1) edge [loop right] node {$\textcolor{red}{a_{11}}$} (s_1)
			(s_2) edge [loop right] node {$\textcolor{red}{a_{22}}$} (s_2)
			(s_0) edge [bend left=15] node {$\textcolor{red}{a_{02}}$} (s_2)
			(s_2) edge [bend left=15] node {$\textcolor{red}{a_{20}}$} (s_0);
			\end{tikzpicture}

			}

			}}
	\subfloat[]{{
		\scalebox{.7}{
			\begin{tikzpicture}[shorten >=1pt,node distance=2.5cm,on grid,auto] 
			\node[state,initial] (q_0)   {$q_0$}; 
			\node[state,accepting] (q_1) [above right=of q_0, label=above:$\textcolor{ForestGreen}{F_1}$]  {$q_1$};
			\node[state,accepting, label=below:$\textcolor{ForestGreen}{F_2}$] (q_2) [below right=of q_0]  {$q_2$};
			\path[->] 
			(q_0) edge [bend left=15] node {$r_1$} (q_1)
			(q_1) edge [bend left=15] node {$r_0$} (q_0)
			(q_0) edge [loop below] node {$r_0$} (q_0)
			(q_1) edge [loop right] node {$r_1$} (q_1)
			(q_2) edge [loop right] node {$r_2$} (q_2)
			(q_0) edge [bend left=15] node {$r_2$} (q_2)
			(q_2) edge [bend left=15] node {$r_0$} (q_0)
			(q_1) edge [bend left=15] node {$r_2$} (q_2)
			(q_2) edge node {$r_1$} (q_1);
			\end{tikzpicture}
			}
			}}
	$\qquad$
	\subfloat[]{{
		\scalebox{.6}{
			\begin{tikzpicture}[shorten >=1pt,node distance=3cm,on grid,auto] 
			\node[state,initial] (s_0)   {$(s_0,q_0)$}; 
			\node[state,accepting] (s_1) [above right=of s_0, label=above:$\textcolor{ForestGreen}{F_1}$]  {$(s_1,q_1)$};
			\node[state] (s_2) [below right=of s_0]  {$(s_0,q_0)$};
			\draw[blue, very thick] (1.2,-3) rectangle (3,-1.2);
			\path (3.65,0) node(x) {\textcolor{blue}{Cycle1}};
			\path (3.65,-2.1) node(x) {\textcolor{blue}{Cycle2}};
			\node[state,accepting] (s_3) [right=of s_1, label=above:$\textcolor{ForestGreen}{F_1}$]  {$(s_1,q_1)$};
			\node[state,accepting] (s_4) [right=of s_2, label=below:$\textcolor{ForestGreen}{F_2}$]  {$(s_2,q_2)$};
			\path[->]
			(s_0) edge node {$\textcolor{red}{a_{01}^p}$} (s_1)
			(s_1) edge [bend right=15] node {$\textcolor{red}{a_{10}^p}$} (s_2)
			(s_2) edge [bend left=15] node {$\textcolor{red}{a_{01}^p}$} (s_3)
			(s_3) edge [bend left=15] node {$\textcolor{red}{a_{10}^p}$} (s_2)
			(s_3) edge [loop right] node {$\textcolor{red}{a_{11}^p}$} (s_3)
			(s_2) edge [bend left=15] node {$\textcolor{red}{a_{02}^p}$} (s_4)
			(s_4) edge [bend left=15] node {$\textcolor{red}{a_{20}^p}$} (s_2)
			(s_4) edge [loop right] node {$\textcolor{red}{a_{22}^p}$} (s_4)
			;
			\end{tikzpicture}
			}
		}}
		\caption{\label{fig:automaton} (a) PL-MDP model with the deterministic label function. (b) LDGBA of LTL formula
		$\varphi_{e}$. (c) The standard product MDP.}
	\end{figure}
